Uncertainty Quantification in Continual Open-World Learning

AI deployed in the real-world should be capable of autonomously adapting to novelties encountered after deployment. Yet, in the field of continual learning, the reliance on novelty and labeling oracles is commonplace albeit unrealistic. This paper addresses a challenging and under-explored problem: a deployed AI agent that continuously encounters unlabeled data - which may include both unseen samples of known classes and samples from novel (unknown) classes - and must adapt to it continuously. To tackle this challenge, we propose our method COUQ "Continual Open-world Uncertainty Quantification", an iterative uncertainty estimation algorithm tailored for learning in generalized continual open-world multi-class settings. We rigorously apply and evaluate COUQ on key sub-tasks in the Continual Open-World: continual novelty detection, uncertainty guided active learning, and uncertainty guided pseudo-labeling for semi-supervised CL. We demonstrate the effectiveness of our method across multiple datasets, ablations, backbones and performance superior to state-of-the-art.

==> sec/2_background.tex <==
\section{Related Works}
\label{sec:background}

\subsection{Uncertainty Quantification}
\subsubsection{Novelty Detection:} Also known as outlier or out-of-distribution (OOD) detection, novelty detection is typically performed by making the network provide an uncertainty score (along with the output) for each input. Uncertainty scores are based on a diverse set of strategies: Softmax score \cite{hendrycks2016baseline} and its temperature scaled variants such as generalized ODIN \cite{liang2018enhancing}, Bayesian networks and ensembles \cite{gal2016dropout}, deep reconstruction or likelihood-based approaches \cite{lee2018simple,ndiour2022subspace}. Most novelty detection methods assume the deployed model has a fixed set of known (old) classes and will not be adapted to post-deployment novelties (e.g. novel classes). Thus, traditional OOD detection is not preoccupied in learning from detected novel data. Rather, they are evaluated and developed to simply detect which samples are novel in a binary partition. 
%Rather, they are evaluated and developed to simply detect which samples are novel in a binary partition. 
% \noindent \textbf{Open-World/Generalized Class Discovery:}
A closely related problem is Open World or Generalized Novel Class Discovery (GCD) first introduced in \cite{vaze2022gcd}. In the GCD setting,  novelties are unknown novel classes that need to be detected and discovered (which and how many) whilst being mixed with unseen samples of the old classes. The objective of GCD, unlike closed-world OOD detection, is to ultimately learn from the identified novel classes. Cite GCD, AGCD. 

\subsubsection{Active Learning:} 
%Explain how uncertainty is quantified and used as informativeness.
% Several semi-supervised solutions \cite{cao2021open, rizve2022openldn, fini2021unified} have been proposed. However, in these semi-supervised methods, different supervision regimes and assumptions lead to solutions that are not easily comparable. For instance, in OpenLDN \cite{rizve2022openldn} supervision is only available for old classes during a given task but not for novel classes, a very different setting then ours, see section \ref{sec:setup}. Moreover, Open-World solutions are not automatically enabled for continual learning, i.e. cannot adapt to novelties several times as needed.
% Most AL methods are offline. AL has a few sampling strategies, including uncertainty-based, diversity-based, etc. 
% Cite AL paper Ranga and get some citations from there. 
Active learning aims to learn from a small set of informative data samples judiciously chosen from a larger unlabeled dataset. There is ample literature on the diverse strategies used for selecting the samples based on uncertainty \cite{lewis_gale,tong_koller} or diversity \cite{brinker}. We refer to \cite{ren_survey_2021,settles2009active} for exhaustive surveys of the methods, which overwhelmingly operate in an offline fashion. The few exceptions to offline AL include active GCD \cite{ma2024active} and GBCL \cite{}.  
%(open-world/GCD setting), GBCL (open world CL setting)...

\subsection{Continual Learning} 
Until now, most works in Continual Learning (CL)  primarily focus on preventing catastrophic forgetting \cite{rios2020lifelong,parisi2019continual} but 
rely on fully supervised data and require the presence of a novelty oracle indicating when the model needs to adapt and providing the labels of the novel data \cite{rios2022incdfm}. Overall, CL solutions have adopted an array of different algorithms to tackle forgetting \cite{kirkpatrick2017overcoming,DBLP:journals/corr/ZenkePG17,rios2018closed,rebuffi2017icarl,wen2021beneficial,cheung2019superposition}.
%including regularization techniques \cite{kirkpatrick2017overcoming,DBLP:journals/corr/ZenkePG17}, replay of past data \cite{rios2018closed,rebuffi2017icarl}, network partitioning and weight masking \cite{wen2021beneficial,cheung2019superposition}, etc. 
Much fewer works \cite{ordisco,Boschini_2022,bagus2022supervised} have proposed solutions to unsupervised or semi-supervised continual learning.
In the semi-supervised setting, models must deal with learning optimally from only a few labeled samples per class, usually employing techniques borrowed from static semi-supervised learning such as pseudo-labeling or label propagation.
%, etc. while also preventing catastrophic forgetting. 
Yet, most current solutions for semi-supervised CL \cite{Boschini_2022} require an oracle to inform the model about incoming novelties and cannot distinguish between old and novel classes. A batch of unlabeled inputs with a mixture of Old and novel class samples is much more challenging since Old classes act as distractors for both novelty detection and pseudo-labeling tasks. 
%of novel class samples. 
% unrealistic for post-deployment adaptation scenarios for which inference on past class samples is still necessary. 
% Because of this these models operate under a far easier learning scenario for which static semi-supervised techniques can be more easily adapted and borrowed. In fact, 
When the oracle is removed, solutions such as \cite{Boschini_2022} no longer work well because their assumptions about the unlabeled samples (as belonging to only novel classes) lead to overconfident predictions and error propagation (see section \ref{sec:results}). 

As a result, OOD methods 
They do not integrate the detected OOD data into the learnt knowledge and thus, have been shown to perform poorly in Continual Learning conditions \cite{rios2022incdfm}. 



% Past CL solutions have largely focused on the forgetting component of continual adaptation but have taken for granted the also very challenging aspect of continual novelty detection. 
% \subsection{Active Learning}

